Inverse Reinforcement Learning in a Continuous State Space with Formal Guarantees

Inverse Reinforcement Learning (IRL) is the problem of finding a reward function which describes observed/known expert behavior. The IRL setting is remarkably useful for automated control, in situations where the reward function is difficult to specify manually or as a means to extract agent preference. In this work, we provide a new IRL algorithm for the continuous state space setting with unknown transition dynamics by modeling the system using a basis of orthonormal functions. Moreover, we provide a proof of correctness and formal guarantees on the sample and time complexity of our algorithm. Finally, we present synthetic experiments to corroborate our theoretical guarantees.

==> 1_introductions.tex <==
\section{Introduction}

Reinforcement learning in the context of a Markov Decision Process (MDP) aims to produce a policy function such that the discounted accumulated reward of an agent following the given policy is optimal.  One difficulty in applying this framework to real world problems is that for many tasks of interest, there is no obvious reward function to maximize.  For example, a car merging onto a highway must account for many different criteria, e.g. avoiding crashing and maintaining adequate speed, and there is not an obvious formula of these variables producing a reward which reflects expert behavior \cite{arora2020survey}.  The Inverse Reinforcement Learning (IRL) problem consists of having as input an MDP with no reward function along with a policy, and the goal is to find a reward function so that the MDP plus the learned reward function is optimally solved by the given policy.   Describing expert behavior in terms of a reward function has been shown to provide a succinct, robust, and interpretable representation of expert behavior for purposes of reinforcement learning \cite{arora2020survey}.

Despite much work over the years, there still exist major limitations in our understanding of IRL.  One major gap is the lack of algorithms for the setting of continuous state space.  This setting is of primary importance  since many promising applications, such as autonomous vehicles and robotics, occur in a continuous setting.  Existing algorithms for IRL in the continuous setting generally do not directly solve the IRL problem, but instead take a policy matching approach which leads to a less robust description of agent preference \cite{arora2020survey}.  Finally, there is a lack of formal guarantees  for IRL methods which make principled understanding of the problem difficult.  

For a comprehensive list of results on the IRL problem, we refer the reader to \cite{arora2020survey} as we next describe works that are closest to ours. Throughout the years, various approaches have been proposed to solve the IRL problem in the continuous state setting. \citet{aghasadeghi2011maximum} used a finite set of parametric basis functions to model the reward function and policy for a policy matching approach.  \citet{boularias2011relative} matched the observed policy while maximizing Relative Entropy and applied this method to continuous tasks through discretization.  \citet{levine2012continuous} maximized the likelihood of the observed policy while representing the reward function as a Gaussian Process.  \citet{finn2016guided} modeled the reward function through a neural network to allow for more expressive rewards. These previous methods rely on heuristic arguments and empirical results to support each approach, but do not provide any theoretical guarantees or the insight that comes with them.  Finally, \citet{komanduru} provided theoretical analysis similar to our work, but only for the discrete IRL setting. 

In contrast to the work above, this paper provides a \textit{formally guaranteed solution} to the IRL problem over a continuous state space when transition dynamics of the MDP are \textit{unknown}.  We accomplish this by representing the estimated transition dynamics as an infinite sum of basis functions from $\mathbb{R}^2 \rightarrow \mathbb{R}$.  Then, under natural conditions on the representations, we prove that a linear program can recover a correct reward function.  We exhibit our main theorem by proving that if the transition functions of the MDP have appropriately bounded partial derivatives and the dynamics are represented over a trigonometric basis, then our algorithm returns a correct reward function with high probability.  However, we emphasize that our results apply under a range of appropriate technical conditions and orthonormal bases.  To the best of our knowledge, we present the first algorithm for IRL in the continuous setting with formal guarantees on correctness, sample complexity, and computational complexity. The total sample and computational complexity of our algorithm depends on the series representations of the transition dynamics over a given basis.  However, if a given set of transition functions can be represented with sufficiently small error over a given basis by a $k \times k$ matrix of coefficients, then our algorithm (see Algorithm \ref{algo:irl}) returns a solution to the IRL problem in $\Ocal(k^2 \log \frac{k}{\delta})$ samples and $\Ocal(k^{2.5})$ arithmetic operations with probability at least $1-\delta$. This sample complexity matches that of the discrete case algorithm of \cite{komanduru}.  For more detailed complexity results, see Section \ref{section:irl}. 


==> checklist.tex <==

\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the Discussions section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{This paper is focused on improving theoretical understanding of IRL in the continuous setting. Potential for harm or benefit will depend on end use-cases.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All results are rigorously proved in the appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Our main contributions are theoretical.  We describe at a high-level how our experiments were completed in Appendix \ref{app:experiments}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{app:experiments}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNo{We only use standard Python libraries for our experiments.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{The data is synthetic.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The data is synthetic.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}{}{}
\end{enumerate}

\end{enumerate}
